Learning and Communications Co-Design for Remote Inference Systems: Feature Length Selection and Transmission Scheduling

In this paper, we consider a remote inference system, where a neural network is used to infer a time-varying target (e.g., robot movement), based on features (e.g., video clips) that are progressively received from a sensing node (e.g., a camera). Each feature is a temporal sequence of sensory data. The inference error is determined by (i) the timeliness and (ii) the sequence length of the feature, where we use Age of Information (AoI) as a metric for timeliness. While a longer feature can typically provide better inference performance, it often requires more channel resources for sending the feature. To minimize the time-averaged inference error, we study a learning and communication co-design problem that jointly optimizes feature length selection and transmission scheduling. When there is a single sensor-predictor pair and a single channel, we develop low-complexity optimal co-designs for both the cases of time-invariant and time-variant feature length. When there are multiple sensor-predictor pairs and multiple channels, the co-design problem becomes a restless multi-arm multi-action bandit problem that is PSPACE-hard. For this setting, we design a low-complexity algorithm to solve the problem. Trace-driven evaluations demonstrate the potential of these co-designs to reduce inference error by up to 10000 times.

==> Contribution.tex <==
The contributions of this paper are summarized as follows:
\begin{itemize}
(1) In this paper, we showed that the inference error is a joint function of the AoI and the feature length of the most recent delivered feature in the receiver. We studied scheduling policies that control the AoI and the feature length to reduce the time-averaged inference error. The scheduling problem for single source is formulated as a semi-Markov decision process (SMDP). We provided two scheduling policies: (i) optimal scheduling policy with time-invariant feature length (TIFL) and (ii) optimal scheduling policy with time-variant feature length (TVFL). The optimal scheduling policy with TIFL minimizes the time-average inference error among the set of causal scheduling policies where the feature length is not allowed to vary over time. On the other hand, optimal scheduling policy with TVFL minimizes the time-average inference error among the set of all causal scheduling policies.  An optimal scheduling policy with TVFL provides the minimum inference error. However, an optimal scheduling policy with TIFL can be useful for reducing switching time and storage cost. This is because if feature length varies over time, neural networks associated with all the choice of feature length need to be stored and switched according to the feature length of the most recent delivered feature. 

(2) We demonstrated that the optimal sending time policy for both time-invariant and time-variant cases is a Gittins index-based threshold policy, where the threshold is equal to the optimal objective value. In the time-invariant case, we computed the optimal objective value using a bisection search algorithm and provided a closed-form expression of the optimal feature length. We obtained the optimal objective value and optimal feature length by using policy iteration algorithm for the SMDP. The policy iteration algorithm can be computationally complex due to high dimension state space and action space. However, we were able to reduce the complexity by leveraging the structure of the optimal sending time.

(3) In addition, we investigated the scheduling policy for the case of multiple sources. This is a challenging problem, as it becomes a multi-arm, multi-action restless bandit problem that is known to be PSPACE-hard. We provide a novel scheduling algorithm for the multiple source scheduling problem. To develop the algorithm, we first decompose the problem into per-source problem by utilizing Lagrangian relaxation. Then, by using the optimal solution to the per-source problem, we provide a method of computing net gain for every choice of feature length for every source. Our scheduling algorithm selects sources and features with maximum net gain that satisfy a channel resource constraint. 

(4) The above scheduling results hold for minimizing any joint function of AoI and feature length. Data driven evaluations show that....


(5) These findings have important implications for the design of real-time inference systems, particularly in the context of IoT applications, where minimizing inference error can have significant impact on system performance.

\end{itemize}

Related work: 
Over the past few years, there has been a rapidly growing body of work using AoI as a metric for scheduling policies in networks

Optimal sampling policies for minimizing non-linear age functions were developed in [13], [15]. Age-optimal transmission scheduling of wireless networks were investigated in, e.g., [18], [19], [25]–[29].

In recent years, the age of information (AoI) has become popular as a metric for sampling and scheduling policies in wireless networks, control system, and remote-estimation. The AoI was first introduced as information freshness metric in \cite{}. Optimal sampling and scheduling policies for minimizing AoI were investigated in \cite{}. In \cite{}, non-linear age functions were studied. However, these works consider monotonic age function. Recently, in \cite{}, it was shown that for a given feature window size or feature length, the inference error can be represented as a function of AoI, where the function can be either monotonic or non-monotonic. The paper \cite{} also studies how to design scheduling policies to minimize the inference error. But, this paper does not analyze the impact of feature window size or feature length on the inference error. In practice, the inference error can be greatly reduced by controlling the feature window. In addition to optimizing AoI, we discuss how to select an optimal feature window to reduce inference error in this current work. 

Multiple source scheduling problem for minimizing time-average inference error is a restless multi-arm bandit (RMAB) problem. The multi-arm restless bandit problem is PSPACE-hard \cite{}. The popular approach to handle the restless-bandit problem is to find the Whittle Index policy \cite{}. Whittle Index policy provides good performance under a certain condition, namely indexability of the RMAB problem. There exists many research works on developing Whittle index policy to minimize linear and non-linear functions of AoI \cite{}. However, the previous works consider monotonic AoI function. Recently, Whittle index for both the monotonic or non-monotonic  functions of AoI is provided in \cite{}. The multiple source scheduling problem in our paper is more complicated than the previous works. Our works is a restless multi-arm bandit multi-action problem with high dimensional and infinite state space. Whittle index policy for multi-action problem is not well-defined. In \cite{}, a modified Whittle index policy is proposed for the multi-action case that also needs to satisfy an indexability condition. In addition to multiple actions, our problem considers high dimensional, infinite state space. The indexability condition is difficult to establish for our problem. Towards this end, we proposed a low-complexity heuristic algorithm that does not require to satisfy any indexability condition. To devise the algorithm, we used a Lagrangian relaxation of the problem which is motivated by the Whittle's approach \cite{}. 

However, there exists much research effort to devise low-complexity and near-optimal algorithms which are largely motivated by Whittle index policy \cite{}. To employ Whittle index policy 

However, Whittle index policies is known to perform well. 

Researcher designed sampling and scheduling policies to minimize linear and non-linear monotonic functions of AoI. Recently, in \cite{}, 

The problem of minimizing age of information was considered in [7] and [8]. In \cite{}, 




\ignore{Whittle index policy is well-know for multi-arm restless bandit problem. However, the Whittle index is not well-defined for multi-arm, multi-action problem.}

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> SystemModel.tex <==


\section{Learning and Communication Co-design: Single Source Case}\label{Scheduling:SingleUser}


\subsection{System Model}\label{SystemModel1}
\begin{figure}[t]
\centering
\includegraphics[width=0.70\textwidth]{Scheduling3.eps}
\caption{\small  A networked real-time supervised learning system, where $X_{t-b}^l:= (V_{t-b}, V_{t-b-1},\ldots, V_{t-b-l+1})$. \label{fig:scheduling}
}
\vspace{-3mm}
\end{figure}
We consider a networked real-time supervised learning system that is composed of a sensor, a transmitter, and a receiver, as illustrated in Fig. \ref{fig:scheduling}. The sensor observes a time-varying target $Y_t \in \mathcal Y$ and feeds its measurements $V_t \in \mathcal V$ to the transmitter. The transmitter progressively generates features $X_{t-b}^l$ from the sensory data $V_t$, where each feature $X_{t-b}^l:= (V_{t-b}, V_{t-b-1},\ldots, V_{t-b-l+1})$ is a temporal sequence taken from $V_t$. For ease of presentation, the temporal sequence length $l$ of feature $X_{t-b}^l$ is called \emph{feature length}. The features are sent one-by-one through a communication channel to the receiver. The receiver provides the most recently received feature to a neural network based predictor that uses the feature to infer the real-time value of $Y_t$. 

\subsubsection{Real-time supervised learning model}
We consider a class of popular supervised learning algorithms called \emph{Empirical Risk Minimization} (ERM) \cite{goodfellow2016deep}. The goal of the ERM is to predict the target $Y_t$ at each time $t$ based on the most recently received feature $X^l_{t-\Delta(t)}=(V_{t-\Delta(t)},$ $V_{t-\Delta(t)-1}, \ldots, V_{t-\Delta(t)-l+1})$, where the \emph{age of information (AoI)} $\Delta(t)$ is the difference between the time stamps of the target $Y_t$ and the freshest observation $V_{t-\Delta(t)}$ in feature $X^l_{t-\Delta(t)}$. In freshness-aware ERM, when $\Delta(t)=\delta$, a neural network associated with AoI $\delta$ and feature length $l$ is trained to construct an output $a=\phi_{l, \delta}(X^l_{t-\delta}) \in \mathcal A$ where $\phi_{l, \delta}: \mathcal V^l \mapsto \mathcal A$ is a function of feature $X^l_{t-\delta} \in \mathcal V^l$ and $\mathcal V^l$ is the set of all $l$-tuples that take values from $\mathcal V$. The performance of the ERM is measured by a loss function $L: \mathcal Y \times \mathcal A \mapsto \mathbb R$, where $L(y, a)$ is the incurred loss if $a \in \mathcal A$ is utilized for inference when $Y_t=y$. The loss function $L$ is determined by the purpose of the supervised learning algorithm. For example, in softmax regression (i.e., neural network based maximum likelihood classification), the output $a=Q_Y$ is a distribution of $Y_t$ and the loss function $L_{\text{log}}(y, Q_Y)=-\text{log}~Q_Y(y)$ is the negative log-likelihood of the value $Y_t=y$. In neural network based mean-squared estimation, a quadratic loss function $L_2(\mathbf y, \mathbf{\hat y})=\|\mathbf y-\mathbf{\hat y}\|^2_2$ is used, where the action $a=\mathbf{\hat y}$ is an estimate of the target value $Y_t=\mathbf y$ and $\| \mathbf y \|_2$ is the $L^2$ or euclidean norm of the vector $\mathbf y$.

Real-time supervised learning consists of two phases: offline training and online inference. In offline training, the neural network is trained using a training dataset denoted by $\{(\tilde Y_0, \tilde X^l_{-\delta})\}$, where $\delta$ is the time difference between the label $\tilde Y_0$ and feature $\tilde X^l_{-\delta}=(\tilde V_{-\delta}, \ldots,$ $ \tilde V_{-\delta-l+1})$.\footnote{We use $\tilde X, \tilde  Y$ to denote the random variables associated to training and use $X, Y$ to denote the random variables for inference.} Let $P_{\tilde Y_0, \tilde X^l_{- \delta}}$ denote the empirical distribution of the label $\tilde Y_0$ and feature $\tilde X_{-\delta}$ in the training dataset, and $\Lambda$ be the set of function mappings from $\mathcal V^l$ to $\mathcal A$ that can be constructed by the neural network. In ERM supervised learning algorithms, the neural network is trained by solving the following stochastic decision problem:   
\begin{align}\label{eq_trainingerror}
\mathrm{err}_{\mathrm{training}}(\delta, l):= \min_{\phi_{l, \delta}\in \Lambda} \mathbb{E}_{Y,X^l \sim P_{\tilde Y_0, \tilde X^l_{-\delta}}}[L(Y,\phi_{l, \delta}(X^l))],
\end{align} 
where $\mathrm{err}_{\mathrm{training}}(\delta, l)$ is the training error. The optimal solution to \eqref{eq_trainingerror} is denoted by $\phi^*_{l, \delta}$. In the online inference phase, the receiver uses the trained neural network $\phi^*_{l, \delta}$ to infer the value of $Y_t$ based on the feature $X^{l}_{t-\delta}$. The expected inference error is given by
\begin{align}\label{instantaneous_err1} 
\mathrm{err}_{\mathrm{inference}}(\delta, l):=\mathbb E_{Y, X^l \sim P_{Y_t, X^{l}_{t-\delta}}}\left[L\left(Y,\phi^*_{l, \delta}(X^l)\right)\right],
\end{align}
where $P_{Y_t, X^{l}_{t-\delta}}$ is the joint distribution of the label $Y_t$ and the feature $X^{l}_{t-\delta}$.

\subsubsection{Joint Impact of AoI and Feature Length on Inference Error}

{\blue Inference error $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ can exhibit a non-monotonic function of AoI $\delta$ for a fixed feature length $l$. A recent work \cite{ShisherMobihoc} conducted five experiments: (a) video prediction, (b) robotic state prediction, (c) actuator state prediction, (d) channel state information prediction, and (e) temperature prediction to show the non-monotonic behavior of inference error with AoI. Furthermore, \cite{ShisherMobihoc} utilizes local information geometric and information-theoretic tools to demonstrate that when the target and feature sequences closely resemble a Markov chain, the inference error becomes a monotonic function of AoI. Conversely, if they deviate from a Markov chain pattern, the inference error becomes non-monotonic with AoI. The paper \cite{ShisherMobihoc} also provides two toy examples which reveal that a stale feature can perform better than a fresh feature if (i) the output of a delayed causal system is predicted based on the input of the system or (ii) the target is correlated with stale features.} 

 \ignore{For a fixed feature length $l$, the relationship between the inference error $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ and the AoI $\delta$ is investigated recently in \cite{ShisherMobihoc}. By using data processing inequality, it is shown that if $Y_t \leftrightarrow X_{t-\mu} \leftrightarrow X_{t-\mu-\nu}$ is a Markov chain for all $\mu, \nu \geq 0$, then $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ increases as the AoI $\delta$ increases. However, if this Markov chain property is not satisfied, the behavior of $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ as a function of AoI $\delta$ may not be monotonic. To quantify the deviation from the Markov chain property, \cite{ShisherMobihoc} proposes an $\epsilon$-Markov chain model denoted by $Y_t \overset{\epsilon}\leftrightarrow X_{t-\mu} \overset{\epsilon}\leftrightarrow X_{t-\mu-\nu}$. Through an information-theoretic analysis and several experiments, the study \cite{ShisherMobihoc} demonstrates that as $\epsilon$ in $Y_t \overset{\epsilon}\leftrightarrow X_{t-\mu} \overset{\epsilon}\leftrightarrow X_{t-\mu-\nu}$ approaches zero for all $\mu, \nu \geq 0$, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ behaves as a non-decreasing function of AoI $\delta$ for the given feature length $l$. However, when $\epsilon$ is large, the function may not be monotonic. The findings suggest that when the target and feature sequences do not follow a Markov chain property, the freshness of features may not guarantee better inference results. In fact, in some experiments, even a stale feature can be a better choice than a fresh feature. For instance, when predicting the output of a delayed causal system based on the input of the system, a stale feature is found to perform better than a fresh feature \cite{ShisherMobihoc}.}

 In Appendix \ref{information-theoreticAnalysis}, we have conducted an information-theoretic analysis to investigate the impact of the feature length $l$ on the inference error $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ for a fixed value of AoI $\delta$. Our analysis reveals that $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ is a non-increasing function of the feature length $l$ for the given AoI $\delta$. This result can be attributed to the fact that by increasing $l$, the feature $X_{t-\delta}^l$ captures more information about $Y_t$, which in turn leads to better inference results. Our information-theoretical analysis is verified by two trace-driven experiments (See Figs. \ref{fig:TrainingCartVelocity}-\ref{fig:Trainingcsi}).



\subsubsection{Communication model}\label{communication}
The system is time-slotted and starts to operate at time slot $t = 0$. At the beginning of each time slot $t$, the sensor observes the target $Y_t \in \mathcal Y$ and generates a sensory output $V_t \in \mathcal V$. For example, $V_t$ can be a noisy measurement of $Y_t$ or a low-dimensional representation extracted from $Y_t$. In time slot $t$, the transmitter appends $V_t$ to a buffer that stores $B$ most recent sensory outputs $(V_t, V_{t-1}, \ldots, V_{t-B+1});$ meanwhile, the oldest output $V_{t-B}$ is removed from the buffer. We assume that the buffer is full initially, such that $B$ signal values $(V_0, V_1, \ldots, V_{-B+1})$ are stored in the buffer at time $t=0$. This ensures that the buffer is always full at any time $t$.\footnote{This assumption does not introduce any loss of generality. If the buffer is no full at time $t=0$, it would not affect our results.} 

In each time slot, the channel is either in an \emph{idle} or \emph{busy} state. If the channel is idle in time slot $t$, the transmitter can select a temporal sequence of sensory data $X_{t-b}^l = (V_{t-b},\ldots,V_{t-b-l+1})$ from the buffer such that $1\leq l\leq B$ and $0\leq b\leq B-l$, and submit the sequence $X_{t-b}^l$ to the channel. In this work, the sequence $X_{t-b}^l$ is called a \emph{feature}. Recall that the temporal sequence length $l$ of feature $X_{t-b}^l$ is called \emph{feature length}. Also, for convenience, the starting position $b$ of feature $X_{t-b}^l$ in the buffer is called \emph{feature position}. This is known as the ``selection-from-buffer" model, which was proposed recently in \cite{ShisherMobihoc}. In contrast to the ``generate-at-will" model \cite{sun2017update, yates2015lazy}, where the transmitter can only select the most recent sensory output $V_t$, the ``selection-from-buffer" model offers greater flexibility by allowing the transmitter to choose multiple values from the buffer, not just the most recent one. When the target and feature sequence is far from a Markov chain, the ``selection-from-buffer" model can potentially achieve better performance than the ``generate-at-will" model. This is because the ``selection-from-buffer" model enables the transmitter to select multiple sensory outputs (which can be stale or fresh) that are relevant to the target $Y_t$. The number of the signal values selected is determined by the feature length. Feature length represents a trade-off between learning and communications: A longer feature can provide better learning performance, whereas it requires more channel resources (e.g., more time slots or more frequency bandwidth) for sending the feature. This motivated us to study a learning-communication co-design problem that jointly optimizes the feature length, feature position, and transmission scheduling.

The feature length and feature position may vary across the features sent over time. Feature transmissions over the channel are non-preemptive: the channel must finish sending the current feature, before becoming available to transmit the next feature. Suppose that the $i$-th feature $X_{S_i-b_i}^{l_i} = (V_{S_i-b_i}, V_{S_i-b_i-1},\ldots, V_{S_i-b_i-l_i+1})$ is submitted to the channel at time slot $t=S_i$, where $l_i$ is its feature length and $b_i$ is its feature position such that $1\leq l_i\leq B$ and $0\leq b_i\leq B-l_i$. It takes $T_i(l_i)\geq 1$ time slots to send the $i$-th feature over the channel such that it is delivered to the receiver at time slot $D_i$, where $S_i < S_i + T_i(l_i) = D_i \leq S_{i+1}$. The feature transmission time $T_i(l_i)$ depends on the feature length $l_i$. Due to time-varying channel conditions, we assume that, given feature length $l_i=l$, the $T_i(l)$'s are \emph{i.i.d.} random variables, with a finite mean $1\leq \mathbb E[T_i(l)] < \infty$. Once a feature is delivered, an acknowledgment (ACK) is sent back to the transmitter, notifying that the channel has become idle. 


In time slot $t$, the $i(t)$-th feature $X_{S_{i(t)}-b_{i(t)}}^{l_{i(t)}}$ is the most recently received feature, where $i(t)=\max_i\{D_i\leq t\}$. The receiver feeds the feature $X_{S_{i(t)}-b_{i(t)}}^{l_{i(t)}}$ to the neural network to infer $Y_t$. \emph{Age of information (AoI)} $\Delta(t)$ is defined as the time difference between the time-stamp of the freshest sensory output $V_{S_{i(t)}-b_{i(t)}}$ in feature $X_{S_{i(t)}-b_{i(t)}}^{l_{i(t)}}$ and the current time $t$, i.e.,  
\begin{align}\label{Def_AoI}
\Delta(t):=t-\max_i \{S_i-b_i: D_i \leq t \}.
\end{align}
Because $D_i < D_{i+1}$, it holds that  
\begin{align}\label{Def_AoI1}
\Delta(t)=t-S_i+b_i,~\text{if}~ D_i \leq t < D_{i+1}.
\end{align}
The initial state of the system is assumed to be $S_0=0, l_0=1, b_0=0, D_0=T_0(l_0)$, and $\Delta(0)$ is a finite constant.
\subsubsection{Freshness-aware learning}
To predict $Y_t$ based on feature $X_{t-\Delta(t)}^{l_{i(t)}}$ and AoI $\Delta(t)$, the receiver employs a trained neural network associated with the AoI $\Delta(t)$ and feature length $l_{i(t)}$. As the receiver uses both feature $X_{t-\Delta(t)}^{l_{i(t)}}$ and it's AoI $\Delta(t)$ to infer $Y_t$, the networked real-time supervised learning system is referred to as \emph{freshness-aware}. Since AoI $\Delta(t)$ and feature length $l_{i(t)}$ can change over time, multiple neural networks need to be trained to cover all possible values of AoI and feature length. AoI can take values from a countably infinite set $\mathbb Z^{+}$. {\blue Usually, when AoI becomes very high, the correlation between the feature and the target weakens significantly. As a consequence, the inference error function tends to approach a maximum point when AoI becomes very high. Consequently, an AoI value, denoted as $D$, can be identified, beyond which the inference error exhibits minimal or no further change. We utilize multiple neural networks $\phi^*_{l, \delta}$ that is trained using \eqref{eq_trainingerror} such that $1\leq l\leq B$ and $1\leq \delta \leq D$. If $\delta > D$, we set $\phi^*_{l, \delta}=\phi^*_{l, D}$.

Another method of freshness-aware learning is to use a wide neural network associated with feature length $l$ that takes AoI as input. To train the wide neural network, the training data samples of all AoI values are combined into a large training dataset and the AoI value is included
in the training data \cite{shisher2021age}. Let $P_{\tilde Y_0, \tilde X^l_{- \Theta}, \Theta}$ denote the empirical distribution of the label $\tilde Y_0$, feature $\tilde X_{-\Theta}$, and AoI $\Theta$ in the training dataset, where the AoI $\Theta \geq 0$ of the feature $\tilde X^l_{- \Theta}$ is the time difference between $\tilde Y_0$ and $\tilde X^l_{- \Theta}$. Denote $\tilde{\Lambda}$ as the set of function mappings from $\mathcal V^l \times \mathbb Z^{+}$ to $\mathcal A$ that can be constructed by the neural network. Then, a neural network with AoI as input is trained using 
$$\min_{\phi_l\in \tilde{\Lambda}} \mathbb{E}_{Y,X,\Theta\sim P_{\tilde Y_0, \tilde X^l_{- \Theta},\Theta}}[L(Y,\phi_l(X,\Theta))].$$}
\ignore{At each time slot $t$, the receiver selects the corresponding neural network associated with the current AoI $\Delta(t)$ and feature length $l_{i(t)}$. To reduce the switching time between networks, we can use a multi-label neural network $\phi^*_{l_{i(t)}}$ that combines all neural networks $\phi^*_{l_{i(t)}, \delta}$ for $\delta=1, 2, \ldots, D$. We utilize the output associated with the current AoI value for inference. If $\Delta(t)$ exceeds the upper bound $D$, we use the output with AoI value $D$ instead.}

Experimental results in \cite[Fig. 6]{shisher2021age} showed that \emph{freshness-aware} supervised learning can achieve better learning performance than \emph{freshness-agnostic} supervised learning, which uses only the feature value $X_{t-\Delta(t)}^{l_{i(t)}}$ to infer $Y_t$. Hence, we consider freshness-aware real-time supervised learning in this paper.  


\ignore{\subsection{Real-time Supervised Learning Model}\label{metrics}
We consider a class of widely used supervised learning algorithms called \emph{Empirical Risk Minimization} (ERM) \cite{goodfellow2016deep}. The goal of the ERM is to predict a target $Y_t$ based on a feature $X^l_{t-\delta}$ that was generated $\delta$ times ago and consists of $l$ consecutive signal values $(V_{t-\delta}, V_{t-\delta-1}, \ldots, V_{t-\delta-l+1})$. In freshness-aware ERM, a neural network associated with AoI $\delta$ and feature length $l$ is trained to construct an output $a=\phi_{l, \delta}(X^l_{t-\delta}) \in \mathcal A$ where $\phi_{l, \delta}: \mathcal X^l \mapsto \mathcal A$ is a function of feature $X^l_{t-\delta} \in \mathcal X^l$ and $\mathcal X^l$ is the set of all $l$-tuple that takes value from the set $\mathcal V$. The performance of ERM is measured by a loss function $L: \mathcal Y \times \mathcal A \mapsto \mathbb R$, where $L(y, a)$ is the incurred loss if $a \in \mathcal A$ is utilized for inference when $Y_t=y$. The loss function $L$ is determined by the purpose of the supervised learning algorithm. For example, in softmax regression (i.e., neural network based maximum likelihood classification), the output $a=Q_Y$ is a distribution of $Y_t$ and the loss function $L_{\text{log}}(y, Q_Y)=-\text{log}~Q_Y(y)$ is the negative log-likelihood of the value $Y_t=y$. In neural network based mean-squared estimation, a quadratic loss function $L_2(\mathbf y, \mathbf{\hat y})=\|\mathbf y-\mathbf{\hat y}\|^2_2$ is used, where the action $a=\mathbf{\hat y}$ is an estimate of the target value $Y_t=\mathbf y$ and $\| \mathbf y \|_2$ is the $L^2$ or euclidean norm of the vector $\mathbf y$.

Real-time supervised learning consists of two phases: offline training and online inference. In offline training, the neural network associated with AoI value $\delta$ and the feature length $l$ is trained using a training dataset denoted by $\{(\tilde Y_0, \tilde X^l_{-\delta})\}$, where the AoI $\delta$ is the time difference between the label $\tilde Y_0$ and feature $\tilde X^l_{-\delta}=(\tilde V_{-\delta}, \ldots,$ $ \tilde V_{-\delta-l+1})$.\footnote{We use $\tilde X, \tilde  Y$ to denote the random variables associated to training and use $X, Y$ to denote the random variables for inference.} Let $P_{\tilde Y_0, \tilde X^l_{- \delta}}$ denote the empirical distribution of the label $\tilde Y_0$ and feature $\tilde X_{-\delta}$ in the training dataset, and $\Lambda$ be the set of function mappings from $\mathcal X^l$ to $\mathcal A$ that can be constructed by the neural network. In ERM supervised learning algorithms, the neural network is trained by solving the following stochastic decision problem:   
\begin{align}\label{eq_trainingerror}
\mathrm{err}_{\mathrm{training}}(\delta, l):= \min_{\phi_{l, \delta}\in \Lambda} \mathbb{E}_{Y,X^l \sim P_{\tilde Y_0, \tilde X^l_{-\delta}}}[L(Y,\phi_{l, \delta}(X^l))],
\end{align} 
where $\mathrm{err}_{\mathrm{training}}(\delta, l)$ is the training error. The optimal solution to \eqref{eq_trainingerror} is denoted by $\phi^*_{l, \delta}$. AoI $\delta$ can take value from the set of natural numbers $\mathbb N$. Because $\mathbb N$ is an infinite set, it is infeasible to train neural networks for all AoI values. Hence, we choose a larger number $D$ such that AoI is rarely greater than $D$ and neural networks are trained by using \eqref{eq_trainingerror} for AoI values $0 \leq \delta \leq D$ and feature length $1 \leq l \leq B$. If $\delta>D$, we consider $\phi^*_{l, \delta}=\phi^*_{l, D}$ for any feature length $l$.

In the online inference phase, the receiver uses a trained neural network $\phi^*_{l{_i(t)}, \Delta(t)}$ at time slot $t$ to infer the value of $Y_t$ based on the feature $X^{l_{i(t)}}_{t-\Delta(t)}$, where $\Delta(t)$ is the AoI and $l_{i(t)}$ is the feature length at time $t$. Let $\mathrm{err}_{\mathrm{inference}}(\Delta(t), l_{i(t)})$ denote the time-average expected inference error at time $t$, where $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ for all $0 \leq \delta \leq D$ and $1 \leq l \leq B$ is defined as
\begin{align}\label{instantaneous_err1} 
\mathrm{err}_{\mathrm{inference}}(\delta, l):=\mathbb E_{Y, X^l \sim P_{Y_t, X^{l}_{t-\delta}}}\left[L\left(Y,\phi^*_{l, \delta}(X^l)\right)\right],
\end{align}
$P_{Y_t, X^{l}_{t-\delta}}$ is the joint distribution of the label $Y_t$ and the feature $X^{l}_{t-\delta}$. 

Because $\Delta(t)$ and $l_{i(t)}$ may vary over time, the neural network needs to be switched accordingly. To reduce the switching time, we can use a multi-label neural network $\phi^*_l$ by combining neural networks $\phi^*_{l, \delta}$ for all $1 \leq \delta \leq D$. The receiver uses the output associated with AoI $\Delta(t)$ at time $t$. If $\Delta(t)>D$, output with the AoI value $D$ is utilized for inference.}

\subsection{Learning and communication co-design problem}
Let $\pi=((S_1, b_1, l_1), (S_2, b_2, l_2), \ldots)$ represent a scheduling policy and $\Pi$ denote the set of all the causal scheduling policies that satisfy the following conditions: (i) the scheduling time $S_i$, the feature position $b_i$, and the feature length $l_i$ are decided based on the current and the historical information available at the transmitter such that $1 \leq l_i \leq B$ and $0 \leq b_i \leq B-l_i$ and (ii) the scheduler has access to the inference error function $\mathrm{err}_{\mathrm{inference}}(\cdot)$ and the distribution of $T_i(l)$ for each $l=1, 2, \ldots, B$. We use $\Pi_{\mathrm{inv}}$ to denote the set of causal scheduling policies with time-invariant feature length, defined as
\begin{align}
 \Pi_{\mathrm{inv}}:=\bigcup_{l=1}^{B} \Pi_l,
\end{align}
where $\Pi_l$ is given by
\begin{align}
\Pi_l:= \{\pi \in \Pi: l_1=l_2=\dots=l\}.
\end{align}
Under policy $\pi$, the time-averaged expected inference error $\bar p_{\pi}$ is given by
\begin{align}
\bar p_{\pi}=\limsup_{T\rightarrow \infty}\frac{1}{T} \mathbb{E}_{\pi} \left[ \sum_{t=0}^{T-1} \mathrm{err}_{\mathrm{inference}}(\Delta(t), l_{i(t)})\right],
\end{align}
where $\mathrm{err}_{\mathrm{inference}}(\Delta(t), l_{i(t)})$ is the expected inference error at time slot $t$.

We consider two problems: (i) The goal of the first problem is to find an optimal policy from $\Pi_{\mathrm{inv}}$ that minimizes the time-averaged inference error and (ii) the second problem is to find an optimal policy from the set of all causal scheduling policies $\Pi$ that minimizes the time-averaged inference error.





==> SystemModel__Md_Kamran_Chowdhury_Shisher_s_conflicted_copy_2023-03-07_.tex <==


\section{System Model, Metric, and Scheduling Policy}


\subsection{System Model}
We consider a time-slotted networked real-time inference system composed of a transmitter and a receiver, as illustrated in Fig. \ref{fig:scheduling}, where the transmitter progressively sends features through a communication channel to the receiver. \ignore{{\blue Based on the feature observations, a neural network in the receiver predicts a time-varying target $Y_t \in \mathcal Y$ .}}

\begin{figure}[t]
\centering
\includegraphics[width=0.70\textwidth]{Scheduling2.eps}
\caption{\small  A networked real-time inference system. \label{fig:scheduling}
}
\vspace{-3mm}
\end{figure}


At the beginning of each time slot $t$, a sensor observes a signal $Y_t \in \mathcal Y$ and generates $V_t \in \mathcal X$. The signal $V_t$ is correlated with $Y_t$. For example, the signal $V_t$ can be a noisy observation of $Y_t$ or a low-dimensional representation of $Y_t$. At every time slot $t$, the sensor appends $V_t$ to a buffer that stores $B$ most recent signal values $(V_t, V_{t-1}, \ldots, V_{t-B+1})$, meanwhile the oldest signal value $V_{t-B}$ is removed from the buffer. The systems starts to operate at time $t=0$ with $B$ signal values $(V_0, V_{-1}, \ldots,$ $ V_{-B+1})$ in the buffer. Let $S_i$ denote the sending time of the $i$-th feature. The $i$-th feature is represented by $X^{l_i}_{S_i-b_i} := (V_{S_i-b_i}, V_{S_i-b_i-1}, \ldots, V_{S_i-b_i-l_i+1})$ that consists of $l_i$ consecutive signal values with the freshest signal value, $V_{S_i-b_i}$, generated at time $S_i-b_i$ and taken from the $b_i$-th position in the buffer. We call $l_i$ and $b_i$ as the feature length and the feature position of the $i$-th feature, respectively. {\blue Let $D_i$ be the delivery time of the $i$-th feature. The $i$-th feature is transmitted by the transmitter at time $S_i$ and takes $T_i(l_i)$ time-slots to be delivered, resulting in a delivery time of $D_i = S_i + T_i(l_i)$. For $l_i=l$, the function $T_i(l) \geq 1$ depends on the feature length $l$ and may vary randomly due to time-varying channel conditions. This paper considers a general function $T_i(l)$ that includes a realistic scenario where longer features may take more time-slots for transmission. We assume that $T_i(l)$'s are i.i.d. with a finite mean $1 \leq \mathbb E[T_i(l)] < \infty$. The receiver sends an acknowledgement (ACK) to the transmitter immediately after the delivery of a feature. Because the ACK is typically a single bit signal, the ACK is assumed to have zero delay.} The system satisfies $0 \leq l_i \leq B$, $0 \leq b_i \leq B-l_i$, and $S_i< D_i \leq S_{i+1}$. The initial state of the system is assumed to be $S_0=0, b_0=0, l_0=1, D_0=T_0(1)$, and $\Delta(0)$ is a finite constant. 

\ignore{After the delivery of the $i$-th feature at time $D_i$, the transmitter inserts a waiting time $Z_{i+1}$ to send the next feature, i.e., $S_{i+1}=D_i+Z_{i+1}$, where $Z_{i+1} \in \{0, 1, \ldots\}$. 
At every $i$-th delivery time $D_i$, a transmission scheduler determines (i) feature length $l_{i+1}$, (ii) feature position $b_{i+1}$, and (iii) a waiting time $Z_{i+1}$ to send $(i+1)$-th feature. Because the scheduler selects feature from a buffer, this model is called ``selection-from-buffer’’ which is proposed recently in \cite{ShisherMobihoc}. }

At time $t$, the generation time of the freshest signal value of the latest received feature is $U(t):=\max_i \{S_i-b_i: D_i \leq t\}$. \emph{Age of information} or simply \emph{AoI} at time $t$ is the time difference between the generation time of the freshest signal value of the latest received feature and the current time, defined as  
\begin{align}\label{Def_AoI}
\Delta(t):=t-U(t)=t-\max_i \{S_i-b_i: D_i \leq t \}.
\end{align}
Because $D_i < D_{i+1}$, $\Delta(t)$ can be also written as 
\begin{align}\label{Def_AoI1}
\Delta(t)=t-U(t)=t-S_i+b_i,~\text{if}~ D_i \leq t < D_{i+1}.
\end{align}
Moreover, at time slot $t$, the length of the latest received feature is $d(t)$, which can be determined by 
\begin{align}\label{feature_length}
d(t)=l_i,~\text{if}~ D_i \leq t < D_{i+1}.
\end{align}

At time $t$, the receiver observes the most recent delivered feature $X^{d(t)}_{t-\Delta(t)}$ and predicts a time-varying target $Y_t$ by using a neural network associated with the AoI $\Delta(t)$ and the feature length $d(t)$. The neural network is trained offline by using a supervised learning algorithm. Supervised learning can be either \emph{freshness-aware} or \emph{freshness-agnostic}. In freshness-aware learning, a neural network is trained to predict $Y_t$ based on the observed feature and its AoI; In freshness-agnostic learning, only the feature is used to predict the target. Our earlier experimental results \cite[Fig. 6]{shisher2021age} suggested that freshness-aware inference can achieve much better performance than freshness-agnostic inference when AoI $\Delta(t)$ varies dynamically over time due to random transmission delay, transmission errors, and  feature processing delay. 

\ignore{Because $1 \leq l_i \leq B$, \eqref{feature_length} implies that the feature length $d(t)$ can take any integer value from $1$ to $B$. In the receiver, $B$ neural networks are available, each trained to handle a different feature length. {\blue At time $t$, the receiver predicts a time-varying target $Y_t$ by using a neural network associated with feature length $d(t)$. If the feature length $d(t)$ changes over time due to varying choices of $l_i$, the receiver must switch to the appropriate neural network.} The receiver can use either freshness-aware or freshness-agnostic methods for real-time inference: In freshness-aware inference, the neural network uses both the feature $X^{d(t)}_{t-\Delta(t)}$ and its AoI $\Delta(t)$ as input, while freshness-agnostic inference only uses the feature $X^{d(t)}_{t-\Delta(t)}$. Our earlier experimental results \cite[Figure 6]{shisher2021age} suggested that freshness-aware inference can achieve much better performance than freshness-agnostic inference when the AoI $\Delta(t)$ varies dynamically over time due to random transmission delay. Hence, we focus on freshness-aware inference in this study. \ignore{At time slot $t$, each of the $B$ neural network takes input $(X^{d(t)}_{t-\Delta(t)}, \Delta(t))$ with zero padding to match the input node of the network. However, only the output from the neural network associated with the feature length $d(t)$ is used to predict $Y_t$.}}


\ignore{At time $t$, the receiver predicts a time-varying target $Y_t$ by using a neural network associated with feature length $d(t)$. The receiver can use either freshness-aware or freshness-agnostic methods for real-time inference: In freshness-aware inference, the neural network uses both the feature $X^{d(t)}_{t-\Delta(t)}$ and its AoI $\Delta(t)$ as input, while freshness-agnostic inference only uses the feature. Our earlier experimental results \cite[Figure 6]{shisher2021age} suggested that freshness-aware inference can achieve much better performance than freshness-agnostic inference when the AoI $\Delta(t)$ varies dynamically over time. Hence, we focus on freshness-aware inference in this study. The feature length $d(t)$ can range from $1$ to $B$ as $1 \leq l_i \leq B$. So, $B$ neural networks must be available in the receiver. At time slot $t$, each neural network takes input $(X^{d(t)}_{t-\Delta(t)}, \Delta(t))$ with zero padding to match the input node of the network. However, only the output from the neural network associated with the feature length $d(t)$ is used to predict $Y_t$.}

\ignore{\subsection{Inference Error}

Let $\phi^*_{l}$ be the trained neural network associated with feature length $l$. The neural network $\phi^*_{l}$ constructs an output action $a=\phi^*(X^l_{t-\Delta(t)}, \Delta(t)) \in \mathcal A$, where $X^l_{t-\Delta(t)} \in \mathcal X^l$ and its AoI $\Delta(t) \in \mathbb N$. The performance of the neural network is measured by a loss function $L: \mathcal Y \times \mathcal A \mapsto \mathbb R$, where $L(y, a)$ is the incurred loss if action $a \in \mathcal A$ is constructed by the neural network when $Y_t=y$. The loss function $L$ is determined by the goal of the inference. For example, in softmax regression (i.e., neural network based maximum likelihood classification), the action $a=Q_Y$ is a distribution of $Y_t$ and the loss function $L_{\text{log}}(y, Q_Y)=-\text{log}~Q_Y(y)$ is the negative log likelihood of the value $Y_t=y$. In neural network based mean-squared estimation, a quadratic loss function $L_2(\mathbf y, \mathbf{\hat y})=\|\mathbf y-\mathbf{\hat y}\|^2$ is used, where the action $a=\mathbf{\hat y}$ is an estimate of the target value $Y_t=\mathbf y$. We assume that for each $l$, $\{(Y_t, X^l_t), t \in \mathbb Z\}$ is a stationary process that is independent of the AoI process $\{\Delta(t), t \in \mathbb Z\}$. This assumptions holds if the sending time of the features does not depend on the process $\{(Y_t, X^l_t), t \in \mathbb Z\}$. For a given AoI value $\Delta(t) = \delta$, the inference error is given by 
\begin{align}\label{instantaneous_err1} 
\mathrm{err}_{\mathrm{inference}}(\delta, l)=\mathbb E_{Y, X \sim P_{Y_t, X^l_{t-\delta}}}\left[L\left(Y,\phi^*_l(X,\delta)\right)\right],
\end{align}
where $P_{Y_t, X^l_{t-\delta}}$ is the joint distribution of the label $Y_t$ and the feature $X^l_{t-\delta}$, and $\phi^*_l$ is the trained neural network function.}

\subsection{Freshness-aware Supervised Learning Model}\label{metrics}
\ignore{The time varying target $Y_t$ is predicted using trained neural networks. A neural network is trained by using a supervised learning algorithm. Supervised learning algorithms can be either \emph{freshness-aware} or \emph{freshness-agnostic}: In freshness-aware supervised learning, both the feature $X^{d(t)}_{t-\Delta(t)}$ and its AoI $\Delta(t)$ are fed to a neural network for predicting $Y_t$; in freshness-agnostic supervised learning, only the feature $X^{d(t)}_{t-\Delta(t)}$ is available at the neural network. Our earlier experimental results \cite[Figure 6]{shisher2021age} suggested that freshness-aware supervised learning can achieve much better performance than freshness-agnostic supervised learning when the AoI $\Delta(t)$ varies dynamically over time. Hence, we focus on freshness-aware supervised learning in this study. Moreover, the feature length $d(t)$ can vary between $1$ and $B$, so $B$ neural networks must be available for each possible feature length.} 

We consider a class of popular supervised learning algorithms called \emph{Empirical Risk Minimization} (ERM) \cite{goodfellow2016deep}. 
In freshness-aware ERM, a neural network associated with feature length $l$ is trained to construct an output action $a=\phi(X^l_{t-\Delta(t)}, \Delta(t)) \in \mathcal A$, where $\phi : \mathcal X^l \times \mathbb N \mapsto \mathcal A$ is a function of feature $X^l_{t-\Delta(t)} \in \mathcal X^l$ and its AoI $\Delta(t) \in \mathbb N$ and $\mathcal X^l$ is the set of all the tuple of $l$ values taken from $\mathcal X$. The performance of ERM is measured by a loss function $L: \mathcal Y \times \mathcal A \mapsto \mathbb R$, where $L(y, a)$ is the incurred loss if action $a \in \mathcal A$ is constructed by the neural network when $Y_t=y$. The loss function $L$ is determined by the goal of the supervised learning algorithm. For example, in softmax regression (i.e., neural network based maximum likelihood classification), the action $a=Q_Y$ is a distribution of $Y_t$ and the loss function $L_{\text{log}}(y, Q_Y)=-\text{log}~Q_Y(y)$ is the negative log likelihood of the value $Y_t=y$. In neural network based mean-squared estimation, a quadratic loss function $L_2(\mathbf y, \mathbf{\hat y})=\|\mathbf y-\mathbf{\hat y}\|^2$ is used, where the action $a=\mathbf{\hat y}$ is an estimate of the target value $Y_t=\mathbf y$.

Real-time supervised learning consists of two phases: offline training and online inference. We will use $\tilde X,\tilde Y$ to denote the random variables associated to training and use $X,Y$ to denote the random variables for inference. In offline training, the neural network associated with AoI value $\delta$ and the feature length $l$ is trained using a training dataset denoted as $\{(\tilde Y_0, \tilde X^l_{-\delta},)\}$, where the training AoI $\delta$ is the time difference between the label $\tilde Y_0$ and feature $\tilde X^l_{-\delta}=(\tilde V_{-\delta}, \ldots,$ $ \tilde V_{-\delta-l+1})$. Training AoI $\delta$ takes value from a finite set $\mathcal D \subset \mathbb N$. Let $P_{\tilde Y_0, \tilde X^l_{- \delta}}$ denote the empirical distribution of the label $\tilde Y_0$, feature $\tilde X_{-\Theta}$, and AoI $\delta$ in the training dataset and $\Lambda$ be the set of functions that maps from $\mathcal X^l \times \mathbb N$ to $\mathcal A$ and can be constructed by the neural network. In ERM algorithms, the training problem is formulated as  
\begin{align}\label{eq_trainingerror}
\mathrm{err}_{\mathrm{training}}(\delta, l):= \min_{\phi\in \Lambda} \mathbb{E}_{Y,X^l \sim P_{\tilde Y_0, \tilde X^l_{-\delta}}}[L(Y,\phi(X^l,\delta))],
%H_L(Y|X) = \min_{\phi} \mathbb{E}_{X,Y\sim P_{Y|X} \otimes P_X}[L(Y,\phi(X))],
\end{align} 
where $\mathrm{err}_{\mathrm{training}}(\delta, l)$ is the minimum training error. The optimal solution to \eqref{eq_trainingerror} is denoted by $\phi^*$.

In online inference, the trained neural network associated with AoI $\Delta(t)$ and the feature length $d(t)$ is employed to predict the target $Y_t$ in real-time based on the recently received feature $X^l_{t-\Delta(t)}$ and {\blue its AoI $\Delta(t)$ is the time difference between the generation time of the freshest signal value $V_{t-\Delta(t)}$ in feature $X^l_{t-\Delta(t)}$ and the current time $t$. We assume that for each $l$, $\{(Y_t, X^l_t), t \in \mathbb Z\}$ is a stationary process that is independent of the AoI process $\{\Delta(t), t \in \mathbb Z\}$. This assumption holds if the sending time of the features does not depend on the process $\{(Y_t, X^l_t), t \in \mathbb Z\}$.} For a given AoI value $\Delta(t) = \delta$, the inference error is given by 
\begin{align}\label{instantaneous_err1} 
\mathrm{err}_{\mathrm{inference}}(\delta, l):=\mathbb E_{Y, X \sim P_{Y_t, X^l_{t-\delta}}}\left[L\left(Y,\phi^*(X,\delta)\right)\right],
\end{align}
where $P_{Y_t, X^l_{t-\delta}}$ is the joint distribution of the label $Y_t$ and the feature $X^l_{t-\delta}$, and $\phi^*$ is the neural network function that was trained by solving \eqref{eq_trainingerror}.

By using information-theoretic analysis and experimental results, the monotonicity of $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ with the AoI $\delta$ and the feature length $l$ is explained in Appendix \ref{information-theoreticAnalysis}. The theoretical and the experimental studies suggest that for a given feature length $l$, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ may not be an increasing function of the AoI $\delta$. It is also observed that for a given AoI $\delta$, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ decreases as the feature length increase, i.e., the longer feature yields better inference. However, longer feature may take longer transmission time that results in higher AoI (See \eqref{Def_AoI1}) and higher AoI may produce higher inference error. Hence, we need to control both the AoI and the feature length intelligently. 

\subsection{Scheduling Policy}
Recall that when a feature is delivered to the receiver, an ACK is sent back to the transmitter with zero delay. This allows the transmitter to know the delivery time $D_i$ of every $i$-th feature. At time $D_i$, a scheduler determines the feature length $l_{i+1}$ and the feature position $b_{i+1}$. The scheduler also inserts a waiting time $Z_{i+1}$ to send the $(i+1)$-th feature such that $S_{i+1}=D_i+Z_{i+1}$. Let $\pi=((Z_1, b_1, l_1), (Z_2, b_2, l_2), \ldots)$ represent a scheduling policy and $\Pi$ denote the set of all the causal scheduling policies that satisfy the following condition: the waiting time $Z_i$, the position of the buffer $b_i$, and the feature length $l_i$ are decided based on the current and the historical information available at the transmitter such that $Z_{i+1} \in \{0, 1, \ldots\}$, $1 \leq l_i \leq B$, and $0 \leq b_i \leq B-l_i+1$. We use $\Pi_1$ to denote the set of causal scheduling policies with time-invariant feature length, defined as
\begin{align}
\Pi_1:=\{ \pi \in \Pi: l_1=l_2=\ldots=l\}.
\end{align}
We assume that the scheduler has access to the distribution of the process $\{(Y_t, X_t), t \in \mathbb Z\}$ but not its realization.

\ignore{\subsection{Problem Formulation} 
As discussed in Section \ref{metrics}, the inference error at time $t$, $\mathrm{err}_{\mathrm{inference}}(\Delta(t), d(t))$, depends on the AoI $\Delta(t)$ and the feature length $d(t)$. Information-theoretic analysis and experiments in Appendix \ref{information-theoreticAnalysis} show that the inference error $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ may not necessarily increase with increasing AoI $\delta$ for a fixed feature length $l$ (See Figs. \ref{fig:TrainingCartVelocity}-\ref{fig:Trainingcsi}), i.e., fresh features do not always guarantee better inference. On the other hand, for a fixed AoI $\delta$, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ decreases with increasing feature length $l$, i.e., longer features yield lower inference error (See Figs. \ref{fig:TrainingCartVelocity}-\ref{fig:Trainingcsi}). However, longer features take longer time to transmit, leading to higher AoI (as per \eqref{Def_AoI1}), and potentially higher inference error.  The increase of AoI may lead to higher inference error. To minimize the long-term average inference error, we need to find an optimal balance between AoI $\Delta(t)$ and feature length $d(t)$. We devise new scheduling algorithms that optimally control AoI $\Delta(t)$ and feature length $d(t)$ to minimize long-term average inference error. 

Let $\pi=((Z_1, b_1, l_1), (Z_2, b_2, l_2), \ldots)$ represent a scheduling policy and $\Pi_1$ be the set of all the causal scheduling policies that satisfy the following condition: the waiting time $Z_i$, the position of the buffer $b_i$, and the feature length $l_i$ are decided based on the current and the historical information available at the transmitter such that $1 \leq l_i \leq B$ and $0 \leq b_i \leq B-l_i+1$. We define $\Pi_2$ as the set of causal policies with time-invariant feature length:
\begin{align}
\Pi_2=\{\pi \in \Pi_1: l_1=l_2=l\ldots\}.
\end{align}

Our goal is to solve two scheduling problems: (i) \emph{Scheduling problem with time-invariant feature length}: In this problem, we need to find an optimal scheduling policy from a set of causal scheduling policies with time-invariant feature length $\Pi_2$;  (ii) \emph{Scheduling problem with time-varying feature length}: In this problem, our objective is to find an optimal scheduling policy from a set of all causal scheduling policies $\Pi_1$, where feature length can be time-varying. The two problems are stated in \eqref{scheduling_problem}. For $j=1, 2$, we need to solve

\begin{align}\label{scheduling_problem}
\bar p_{opt, j}=\inf_{\pi \in \Pi_j}  \limsup_{T\rightarrow \infty}\frac{1}{T} \mathbb{E}_{\pi} \left[ \sum_{t=0}^{T-1} \mathrm{err}_{\mathrm{inference}}(\Delta(t), d(t))\right], 
\end{align}
where $\mathrm{err}_{\mathrm{inference}}(\Delta(t), d(t))$ is the inference error at time slot $t$, $\bar p_{opt, 1}$ is the optimum objective value of the scheduling problem with time-varying feature length, and $\bar p_{opt, 2}$ is the optimum objective value of the scheduling problem with time-invariant feature length.  

The scheduling problem \eqref{scheduling_problem} can be equivalently expressed as an infinite time-horizon average-cost semi-Markov decision process (SMDP) with two-dimensional state space and three-dimensional action space, as detailed in Appendix \ref{SMDP}. The problem complexity arises from the fact that it is an an infinite horizon SMDP with large number of states and actions. This problem is more challenging than the problems addressed in previous studies such as \cite{SunNonlinear2019, sun2017update, kosta2017age, ShisherMobihoc}, which were either MDPs or SMDPs with one dimensional state and one or two dimensional action spaces.

\begin{remark}
{\normalfont Because $\Pi_2 \subset \Pi_1$, the optimal scheduling policy with time-varying feature length leads to lower inference error compared to the optimal scheduling policy with time-invariant feature length, but requires more storage for multiple neural networks. Moreover, scheduling policy with time-varying feature length needs time for switching a neural network which may not be feasible in some applications. As a result, the scheduling problem with time-invariant feature length may be more practical. Thus, two scheduling problems are considered in this paper.}
\end{remark}}

\ignore{A network takes feature $X^{d(t)}_{t-\Delta(t)}$ and its AoI $\Delta(t)$ as inputs to predict $Y_t \in \mathcal Y$. The feature $X^l_{t}=(V_{t}, V_{t-1}, \ldots, V_{t-l+1})$ is a time sequence of length $l$ made up of signal values $V_t$ from the finite space $\mathcal X$. The feature length $d(t)$ can vary between $1$ and $B$, so $B$ neural networks must be available for each possible length.} 

\ignore{\section{System Model for Real-time Inference}
\begin{figure}[h]
  \centering
  
\includegraphics[width=0.65\textwidth]{LearningModel1.eps}
\caption{\small A system model for real-time inference. \label{fig:learning}}
\end{figure}

{\blue We consider the real-time inference system illustrated in Fig. \ref{fig:learning}. The objective of the system is to infer a time-varying target $Y_t \in \mathcal Y$ based on a feature $X^l_{t-\Delta(t)}$ which is sent from a sensor through a communication channel. A neural network takes the feature $X^l_{t-\Delta(t)}$ as an input to infer the target $Y_t \in \mathcal Y$. Each feature $X^l_{t}=(V_{t}, V_{t-1}, \ldots, V_{t-l+1})$ is a time sequence with length $l$, where $V_t$ is a signal value generated by the sensor at time $t$. The signal $V_t$ takes a value from the finite space $\mathcal X$ and the feature $X^l_{t}$ takes value from $\mathcal X^l$, which is the set of all $l$ tuples of numbers taken from $\mathcal X$.} The time-sequence length $l$ of feature $X^l_{t-\Delta(t)}$ is called \emph{feature length}. The Age of information (AoI) $\Delta(t)$ represents the time difference $\Delta(t)$ between the generation time of the freshest signal value $V_{t-\Delta(t)}$ in feature $X^l_{t-\Delta(t)}$ and the current time $t$. The AoI $\Delta(t)$ can vary dynamically over time due to random transmission errors and communication delays. 

The neural network is trained by using a supervised learning algorithm. Supervised learning algorithms can be either \emph{freshness-aware} or \emph{freshness-agnostic}: In freshness-aware supervised learning, both the feature $X^l_{t-\Delta(t)}$ and its AoI $\Delta(t)$ are fed to a neural network for predicting $Y_t$; in freshness-agnostic supervised learning, only the feature $X^l_{t-\Delta(t)}$ is available at the neural network. Our earlier experimental results \cite[Figure 6]{shisher2021age} suggested that freshness-aware supervised learning can achieve much better performance than freshness-agnostic supervised learning when the AoI $\Delta(t)$ varies dynamically over time. Hence, we focus on freshness-aware supervised learning in this study. 

We consider a class of popular supervised learning algorithms called \emph{Empirical Risk Minimization} (ERM) \cite{goodfellow2016deep}. In freshness-aware ERM algorithms, the neural network is trained to construct an output action $a=\phi(X^l_{t-\Delta(t)}, \Delta(t)) \in \mathcal A$, where $\phi : \mathcal X^l \times \mathcal D \mapsto \mathcal A$ is a function of feature $X^l_{t-\Delta(t)} \in \mathcal X^l$ with length $l$ and its AoI $\Delta(t) \in \mathcal D$ \footnote{{\blue AoI $\Delta(t)$ can take values from a set of natural numbers $\mathbb N$, which is countably infinite. However, large AoI value rarely occurs and insignificant in practice. Hence, we consider a finite set $\mathcal D=\{0, 1, \ldots, D\} \subset \mathbb N$, which is upper bounded by $D$.}}. The performance of ERM is measured by a loss function $L: \mathcal Y \times \mathcal A \mapsto \mathbb R$, where $L(y, a)$ is the incurred loss if action $a \in \mathcal A$ is constructed by the neural network when $Y_t=y$. We assume that $\mathcal Y$ and $\mathcal X^l$ are discrete and finite sets. The loss function $L$ is determined by the goal of the supervised learning algorithm. For example, in softmax regression (i.e., neural network based maximum likelihood classification), the action $a=Q_Y$ is a distribution of $Y_t$ and the loss function $L_{\text{log}}(y, Q_Y)=-\text{log}~Q_Y(y)$ is the negative log likelihood of the value $Y_t=y$. In neural network based mean-squared  estimation, a quadratic loss function $L_2(\mathbf y, \mathbf{\hat y})=\|\mathbf y-\mathbf{\hat y}\|^2$ is used, where the action $a=\mathbf{\hat y}$ is an estimate of the target value $Y_t=\mathbf y$.

\subsection{Offline Training Error and Online Inference Error}
Real-time supervised learning consists of two phases: offline training and online inference. We will use $\tilde X,\tilde Y$ to denote the random variables associated to training and use $X,Y$ to denote the random variables for inference. In offline training, the neural network is trained using a training dataset denoted as $\{(\tilde Y_0, \tilde X^l_{-\Theta})\}$, where the training AoI $\Theta$ is the time difference between the label $\tilde Y_0$ and feature $\tilde X^l_{-\Theta}=(\tilde V_{-\Theta}, \ldots,$ $ \tilde V_{-\Theta-l+1})$ for training. {\blue The AoI $\Delta(t)$ can take values from a finite set $\mathcal D$. In order to train a neural network for multiple AoI values, a training dataset $\{(\tilde Y_0, \tilde X^l_{-\Theta})\}$ is prepared with a finite set of training AoI values $\mathcal D$.} For a given AoI value $\Theta=\delta$, the training error of a freshness-aware ERM algorithm is determined as 
\begin{align}\label{eq_trainingerror}
\mathrm{err}_{\mathrm{training}}(\delta, l) = \min_{\phi \in \Lambda} \mathbb{E}_{Y,X\sim P_{\tilde Y_0, \tilde X^l_{-\delta}}}[L(Y,\phi(X,\delta))],
\end{align} 
where $P_{\tilde Y_0, \tilde X^l_{-\delta}}$ is the joint empirical distribution of the label $\tilde Y_0$ and the feature $\tilde X^l_{-\delta}$ in the training dataset, and $\Lambda$ is the set of functions that map from $\mathcal X^l \times \mathcal D$ to $\mathcal A$ and can be constructed by neural networks. Let $\phi^*_{P_{\tilde Y_0, \tilde X^l_{-\delta}}}$ denote the optimal solution to \eqref{eq_trainingerror}.

In online inference, the trained neural network is employed to predict the target $Y_t$ in real-time, based on the recently received feature $X^l_{t-\Delta(t)}$ and {\blue its AoI $\Delta(t)$ is the time difference between the generation time of the freshest signal value $V_{t-\Delta(t)}$ in feature $X^l_{t-\Delta(t)}$ and the current time $t$. We assume that for each $l$, $\{(Y_t, X^l_t), t \in \mathbb Z\}$ is a stationary process that is independent of the AoI process $\{\Delta(t), t \in \mathbb Z\}$. This assumptions holds if the sending time of the features does not depend on the process $\{(Y_t, X^l_t), t \in \mathbb Z\}$.} For a given AoI value $\Delta(t) = \delta$, the inference error is given by 
\begin{align}\label{instantaneous_err1} 
\mathrm{err}_{\mathrm{inference}}(\delta, l)=\mathbb E_{Y, X \sim P_{Y_t, X^l_{t-\delta}}}\left[L\left(Y,\phi^*_{P_{\tilde Y_0, \tilde X^l_{-\delta}}}(X,\delta)\right)\right],
\end{align}
where $P_{Y_t, X^l_{t-\delta}}$ is the joint distribution of the label $Y_t$ and the feature $X^l_{t-\delta}$, and $\phi^*_{P_{\tilde Y_0, \tilde X^l_{-\delta}}}$ is the neural network function that was trained by solving \eqref{eq_trainingerror}.}
%In online inference phase, the length of the feature $d_t$ can be time varying. Hence, a set of neural network functions $\{\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}: d \in \mathcal L\}$ is used to predict the target in $Y_t$. At time slot $t$, if the length of the feature is $d_t=d$, then the neural network function $\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}$ is used. We assume that for all $d \in \mathcal L$, $\{(Y_t , X_{t, d} ), t \in \mathbb Z\}$ is a stationary process that is independent of the inference AoI process $\{\Delta_t, t \in \mathbb Z\}$. Given $\Delta_t=\delta$ and $d_t=d$, the expected inference error in time slot $t$ is given by
%\begin{align}\label{instantaneous_err1} 
%p(\delta, d)=\mathbb E_{Y, X \sim P_{Y_t, X_{t-\delta, d}}}\left[L\left(Y,\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}(X,\delta)\right)\right],
%\end{align}
%where $P_{Y_t, X_{t-\delta, d}}$ is the distribution of the inference label $Y_t$ and the feature $X_{t-\delta, d}$. The time-average expected inference error during the time slots $t=0,1,\ldots, T-1$ is given by
%\begin{align}\label{eq_inferenceerror}
%\mathrm{err}_{\mathrm{inference}}(T)= \frac{1}{T} \mathbb E \left [ \sum_{t=0}^{T-1} p(\Delta_t, d_t)\right].
%\end{align}


%By using information-theoretic approximations and experimental studies, we observe that for a given length $l$, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ may not be a monotonic function of AoI $\delta$,. Even the fresh feature (AoI=0) may not be better \cite{ShisherMobihoc}. On the other hand, $\mathrm{err}_{\mathrm{inference}}(\delta, l)$ decreases as the length $l$ increases. However, transmission time of the feature increases as the length of the feature increases. Also, the AoI of the feature increases as the transmission time increases. Hence, it is not always beneficial to transmit a feature with large length. So, to reduce the inference error, we need to devise scheduling algorithms that controls the AoI and the length of the feature intelligently.

%This explains the experimental results in Fig. \ref{fig:TrainingCartVelocity}, which depicts the performance of the actuator state prediction. We consider a CartPole-v1 task, which is solved by using Deep Q Network (DQN) algorithm. We simulated the CartPole-v1 environment for $10^4$ episodes and collected time-series dataset that contains the pole angle $Y_t$ and the velocity of the cart $x_{t}$. The pole angle at time slot $t$ is predicted based on a vector of cart velocity $X_{t-\delta, d}=(x_{t-\delta}, x_{t-\delta-1}, \ldots, x_{t-\delta-d+1})$ with feature length $d$ and AoI $\delta$. As observed in Fig. \ref{fig:TrainingCartVelocity}. the training error and the inference error decreases as the length of the feature increases. Also, as illustrated in the Fig. \ref{fig:TrainingCartVelocity}, the training error and the inference error may not be monotonic functions of AoI.



% Because $\tilde Y_0 \leftrightarrow  \tilde X_{-\Theta, d_1} \leftrightarrow  \tilde X_{-\Theta, d_2}$ is a Markov chain for all $1 \leq d_2 \leq d_1$, one can prove Lemma \ref{lemma1} by using data processing inequality \cite{Dawid2004} for Markov chain. 
 
%\subsection{Offline Training Error}
%The real-time supervised learning system consists of two phases: (i) Offline training and (ii) Online inference.  In the offline training phase, the neural network is trained using a training dataset. Let $P_{\tilde Y_0, \tilde X_{-\Theta, d}, \Theta}$ denote the empirical distribution of the label $\tilde Y_0$, feature $\tilde X_{-\Theta, d}$, and AoI $\Theta$ in the training dataset, where $d \in \mathcal L$ is the length of the feature and the AoI $\Theta \geq 0$ of the feature $\tilde X_{-\Theta, d}$ is the time difference between $\tilde Y_0$ and $\tilde X_{-\Theta, d}$. In ERM algorithms, the  training problem is formulated as  
%\begin{align}\label{eq_trainingerror}
%\mathrm{err}_{\mathrm{training}}(\Theta, d) = \min_{\phi_d \in \Lambda_d} \mathbb{E}_{Y,X,\Theta\sim P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}[L(Y,\phi(X,\Theta))],
%%H_L(Y|X) = \min_{\phi} \mathbb{E}_{X,Y\sim P_{Y|X} \otimes P_X}[L(Y,\phi(X))],
%\end{align} 
%where $\Lambda_d$ is the set of functions that can be constructed by the neural
%network, and $\mathrm{err}_{\mathrm{training}}(\Theta, d)$ is the minimum training error. The optimal solution to \eqref{eq_trainingerror} is denoted by $\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}$.
%
%Let $\Phi_d=\{\phi_d : \mathcal X_d \times \mathcal D \mapsto \mathcal A\}$ be the set of all functions mapping
%from $\mathcal X_d \times \mathcal D$ to $\mathcal A$. Any action $\phi_d(X_d,\theta)$ constructed by the neural network belongs to $\Phi_d$, whereas the neural network cannot produce some functions in $\Phi_d$. Hence, $\Lambda_d \subseteq \Phi_d$. By relaxing the feasible set $\Lambda_d$ in \eqref{eq_trainingerror} as $\Phi_d$, we obtain a lower bound of $\mathrm{err}_{\mathrm{training}}(\Theta, d)$, i.e.,
%\begin{align}\label{eq_TrainingErrorLB}
%H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)=\min_{\phi_d \in \Phi_d} \mathbb{E}_{Y,X,\Theta\sim P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}[L(Y,\phi_d(X,\Theta))], 
%\end{align} 
%where $H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)$ is a generalized conditional entropy of $\tilde Y_0$ given $(\tilde X_{-\Theta, d},\Theta)$ \cite{Dawid2004, Dawid1998,farnia2016minimax}. 
%Compared to $\mathrm{err}_{\mathrm{training}}$, its information-theoretic lower bound $H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)$ is mathematically more convenient to analyze. For notational convenience, in \cite{ShisherMobihoc} $H_L(\tilde Y_0| \tilde X_{-\Theta},\Theta)$ is referred as an \emph{L-conditional entropy}, because it is associated with a loss function $L$. The gap between $\mathrm{err}_{\mathrm{training}}$ and the lower bound $H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)$ was studied recently in \cite{shisher2022local}, where the gap is small if the function spaces $\Lambda_d$ and $\Phi_d$ are close to each other, e.g., when the neural network is sufficiently wide and deep \cite{goodfellow2016deep}. 
%
%The \emph{$L$-entropy} of a random variable $Y$ is defined as \cite{Dawid2004, farnia2016minimax}
%\begin{align}\label{eq_Lentropy}
%H_L(Y) = \min_{a\in\mathcal A} \mathbb{E}_{Y \sim P_{Y}}[L(Y,a)].
%\end{align} 
%Let $a_{P_Y}$ denote an optimal solution to \eqref{eq_Lentropy}, which is called a \emph{Bayes action} \cite{Dawid2004}.
%The $L$-conditional entropy of $Y$ given $X=x$ is 
%\begin{align}\label{given_L_condentropy}
%H_L(Y| X=x)= \min_{a \in\mathcal A}\! \mathbb E_{Y\sim P_{Y| X=x}} [L(Y, a)].
%\end{align}
%Using \eqref{given_L_condentropy}, we can get the $L$-conditional entropy of $Y$ given $X$ \cite{Dawid2004, farnia2016minimax}
%\begin{align}\label{eq_cond_entropy1}
%H_L(Y|X)=\sum_{x \in \mathcal X} P_X(x) H_L(Y| X=x).
%\end{align}
%Similar to \eqref{eq_cond_entropy1}, \eqref{eq_TrainingErrorLB} can be decomposed as
%\label{eq_TrainingErrorLB1}
%\begin{align}\label{eq_TrainingErrorLB1}
%\!\!\!H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)=\sum_{\substack{x_d \in \mathcal X_d, \theta \in \mathcal D}} \!\!\!\! P_{\tilde X_{-\Theta, d}, \Theta}(x_d, \theta) H_L(\tilde Y_0|\tilde X_{-\theta, d}=x_d, \Theta=\theta).\!\!\!
%\end{align}

%We assume that in the training dataset, the AoI $\Theta$ is independent of the label $\tilde Y_0$ and feature $\tilde X_{-\mu}$ for all $\mu\geq 0$. Then, one can get for all $d \in \mathcal L$
%\begin{align}\label{freshness_aware_cond}
%\!\! H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)\!\overset{(a)}{=}&\sum_{\substack{x_d \in \mathcal X_d, \theta \in \mathcal D}} P_{\tilde X_{-\Theta, d}, \Theta}(x_d, \theta) H_L(\tilde Y_0|\tilde X_{-\theta, d}=x_d, \Theta=\theta)\nonumber\\
%\overset{(b)}{=}&\sum_{\substack{x_d \in \mathcal X_d, \theta \in \mathcal D}} P_{\tilde X_{-\Theta, d}, \Theta}(x_d, \theta) H_L(\tilde Y_0|\tilde X_{-\theta, d}=x_d)\nonumber\\
%\overset{(c)}{=}&\sum_{\substack{x_d \in \mathcal X_d, \theta \in \mathcal D}} P_{\tilde X_{-\theta, d}}(x_d)P_{ \Theta}(\theta) H_L(\tilde Y_0|\tilde X_{-\theta, d}=x_d)\nonumber\\
%\overset{(d)}{=}&\sum_{\theta \in \mathcal D} P_{\Theta}(\theta) \sum_{x_d \in \mathcal X_d} P_{\tilde X_{-\theta, d}}(x_d) H_L(\tilde Y_0|\tilde X_{-\theta, d}=x_d)\nonumber\\
%\overset{(e)}{=}&\sum_{\theta \in \mathcal D} P_{\Theta}(\theta)~H_L(\tilde Y_0| \tilde X_{-\theta, d}),
%\end{align}
%where the equality (a) is obtained from the definition \eqref{eq_TrainingErrorLB1}, (b) and (c) hold due to the assumption that the AoI $\Theta$ is independent of the label $\tilde Y_0$ and feature $\tilde X_{-\mu}$ for all $\mu\geq 0$, rearranging (c), we get (d), and (e) is obtained by the definition \eqref{eq_cond_entropy1} of $L$-conditional entropy.
%
%By choosing different $L$ in \eqref{eq_Lentropy}, a broad class of $L$-entropies is obtained. In particular, Shannon’s entropy is derived if $L$ is the logarithmic loss function $L_{\log}(y,Q_{Y}) = - \log Q_{Y}(y)$. More examples of the loss function $L$, the definitions of $L$-divergence $D_L(P_Y || Q_Y)$, $L$-mutual information $I_L(Y; X)$, and $L$-conditional mutual information $I_L(Y; X| Z)$ are provided in \cite{technical_report}. In general, $I_L( X ; Y)  \neq I_L(Y ; X)$, which is different from $f$-mutual information. Moreover, a comparison among the $L$-divergence, Bregman divergence \cite{dhillon2008matrix}, and the $f$-divergence \cite{csiszar2004information} is provided in \cite{technical_report}.
%
%
%%The $L$-\emph{divergence} $D_L(P_{Y} || P_{\tilde Y})$ of $P_{Y}$ from $P_{\tilde Y}$ can be expressed as \cite{Dawid2004, farnia2016minimax}
%%\begin{align}\label{divergence}
%%   \!\!\!\!\!\! D_L(P_{Y} || P_{\tilde Y})\!=\!\mathbb E_{Y \sim P_{\tilde Y}}\left[L\left(Y, a_{P_{Y}}\right)\right]-\mathbb E_{Y \sim P_{\tilde Y}}\left[L\left(Y, a_{P_{\tilde Y}}\right)\right] \geq 0.
%%%    =&H_L(\tilde Y; Y)-H_L(\tilde Y)\geq 0.
%%\end{align}
%%The \emph{$L$-mutual information} $I_L(Y;X)$ is defined as \cite{Dawid2004, farnia2016minimax}
%%\begin{align}\label{MI}
%%I_L(Y; X)=& \mathbb E_{X \sim P_{X}}\left[D_L\left(P_{Y|X}||P_{Y}\right)\right]\nonumber\\
%%=&H_L(Y)-H_L(Y|X) \geq 0,
%%\end{align}
%%which measures the performance gain in predicting $Y$ by observing $X$. In general, $I_L(Y;X)$ $\neq$ $I_L(X;Y)$. The $L$-conditional mutual information $I_L(Y; X | Z)$ is given by 
%%\begin{align}\label{CMI}
%%I_L(Y; X|Z)=& \mathbb E_{X, Z \sim P_{X, Z}}\left[D_L\left(P_{Y|X, Z}||P_{Y | Z}\right)\right]\nonumber\\
%%=&H_L(Y | Z)-H_L(Y|X, Z).
%%\end{align}
%%
%
%\subsection{Online Inference Error}
%In the online inference phase, $|\mathcal L|$ neural predictors $\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}$ for all $d \in \mathcal L$ are used to predict the target $Y_t$ in real-time. For a given $d \in \mathcal L$, a neural prediction $\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}$ is trained by \eqref{eq_trainingerror}. We assume that for all $d \in \mathcal L$, $\{(Y_t , X_{t, d} ), t \in \mathbb Z\}$ is a stationary process that is independent of the AoI process $\{\Delta_t, t \in \mathbb Z\}$. Using this assumption, the time-average expected inference error during the time slots $t=0,1,\ldots, T-1$ is given by
%\begin{align}\label{eq_inferenceerror}
%\mathrm{err}_{\mathrm{inference}}(T)= \frac{1}{T} \mathbb E \left [ \sum_{t=0}^{T-1} p(\Delta_t, d_t)\right],
%\end{align}
%where \begin{align}\label{instantaneous_err1} 
%p(\delta, d)=\mathbb E_{Y, X \sim P_{Y_t, X_{t-\delta, d}}}\left[L\left(Y,\phi^*_{P_{\tilde Y_0, \tilde X_{-\Theta, d},\Theta}}(X,\delta)\right)\right],
%\end{align}
%$p(\Delta_t, d_t)$ is the expected inference error in time slot $t$, $d_t$ is the feature length, and $\Delta_t$ is the inference AoI at time $t$, i.e., the time difference between label $Y_t$ and feature $X_{t-\Delta_t. d_t}$. 
%
%Now, we define $L$-cross entropy between distributions $P_Y$ and $P_{\tilde Y}$ as 
%\begin{align}\label{CrossEntropyEqn}
%H_L(P_Y; P_{\tilde Y})= \mathbb E_{Y \sim P_Y}[L(Y, a_{P_{\tilde Y}})],
%\end{align}
%where $a_{P_{\tilde Y}}$ is the Bayes action associated with distribution $P_{\tilde Y}$. Replacing $P_Y$ and $P_{\tilde Y}$ in \eqref{CrossEntropyEqn} with $P_{Y|X=x}$ and $P_{\tilde Y|\tilde X=x}$, respectively, we obtain $L$-conditional cross entropy between distributions $P_{Y|X=x}$ and $P_{\tilde Y|\tilde X=x}$ as 
%\begin{align}\label{CondCrossEntropyEqn}
%H_L(P_{Y|X=x}; P_{\tilde Y|\tilde X=x})= \mathbb E_{Y \sim P_{Y|X=x}}[L(Y, a_{P_{\tilde Y|\tilde X=x}})].
%\end{align}
%Furthermore, the $L$-conditional cross entropy between distributions $P_{Y|X}$ and $P_{\tilde Y|\tilde X}$ is given by, 
%\begin{align}\label{CondCrossEntropyEqnG}
%H_L(P_{Y|X}; P_{\tilde Y|\tilde X})= \sum_{x \in \mathcal X} \mathbb E_{Y \sim P_{Y|X=x}}[L(Y, a_{P_{\tilde Y|\tilde X=x}})].
%\end{align}
%If the neural network in \eqref{instantaneous_err1} is replaced by the Bayes action $a_{P_{\tilde Y_0|\tilde X_{-\delta, d}=x_d}}$, then the inference error $p(\delta)$ becomes an $L$-conditional cross entropy
%\begin{align}\label{inferenceConditionCross}
%H_L(P_{Y_t|X_{t-\delta, d}}; P_{\tilde Y_0|\tilde X_{-\delta, d}})= \sum_{x_d \in \mathcal X_d} \mathbb E_{Y \sim P_{Y_t|X_{t-\delta, d}=x_d}}[L(Y, a_{P_{\tilde Y_0|\tilde X_{-\delta, d}=x_d}})].
%\end{align}
%
%If the set of functions $\Lambda_d$ and $\Phi_d$ are close to each other, the difference between $p(\delta, d)$ and $H_L(P_{Y_t|X_{t-\delta, d}}; P_{\tilde Y_0|\tilde X_{-\delta, d}})$ is small. 

%\subsection{Impact of Length of Features on Training Error and Inference Error}
%In this section, we will study how the length of the feature $d$ affects the $L$-conditional entropy $H_L(\tilde Y_0| \tilde X_{-\Theta, d}, \Theta)$, which is the lower bound of the training error. We will also analyze the impact of the length of the feature $d$ on the $L$-conditional cross entropy $H_L(P_{Y_t|X_{t-\delta, d}}; P_{\tilde Y_0|\tilde X_{-\delta, d}})$.  
%\subsubsection{Training Error vs. Length of the Feature}
%\begin{lemma}
%The $L$-conditional entropy $H_L(\tilde Y_0| \tilde X_{-\Theta, d}, \Theta)$ is a non-increasing function of the length of the feature $d$.
%\end{lemma}
%\begin{proof}
%From \eqref{freshness_aware_cond}, we obtain
%\begin{align}\label{freshness_aware_cond}
%\!\! H_L(\tilde Y_0| \tilde X_{-\Theta, d},\Theta)\!=\sum_{\theta \in \mathcal D} P_{\Theta}(\theta)~H_L(\tilde Y_0| \tilde X_{-\theta, d}).
%\end{align}
%Recall that $\tilde X_{-\theta, d}=(\tilde x_{-\theta}, \tilde x_{-\theta-1}, \ldots, \tilde x_{-\theta-d_1+1})$. For all $1 \leq d_1 \leq d_2$, the feature $\tilde X_{-\theta, d_2}$ consists of $\tilde X_{-\theta, d_1}$ and $(\tilde x_{-\theta-d_1}, \ldots, \tilde x_{-\theta-d_2+1})$. Hence, $\tilde Y_0 \leftrightarrow \tilde X_{-\theta, d_2} \leftrightarrow \tilde X_{-\theta, d_1}$ is a Markov chain. Now, we use the following data processing inequality for $L$-conditional entropy.
%\begin{lemma}\label{DataprocessingEn}
%If $Y \leftrightarrow X \leftrightarrow Z$ is a Markov chain, then 
%\begin{align}\label{datainequality}
%H_L(Y|X) \leq H_L(Y|Z).
%\end{align}
%\end{lemma}
%\begin{proof}
%By using the definition of $L$-conditional mutual information $I_L(Y; Z|X)$, we get 
%\begin{align}\label{inequality}
%H_L(Y|X, Z)=&H_L(Y|Z)-I_L(Y; X|Z) \nonumber\\
%\leq&H_L(Y|Z),
%\end{align}
%where the last inequality holds because $I_L(Y; X|Z) \geq 0$.
%Let $ \Phi=\{f : \mathcal X \times \mathcal Z \mapsto \mathcal A\}$ be the set of all functions mapping
%from $\mathcal X \times \mathcal Z$ to $\mathcal A$. Also, Let $ \Psi=\{g : \mathcal X \mapsto \mathcal A\}$ be the set of all functions mapping
%from $\mathcal X$ to $\mathcal A$. Given a function $f \in \Phi$, for all $x \in \mathcal X$, and $z \in \mathcal Z$, define
%\begin{align}
%\alpha(x, z)=\sum_{y \in \mathcal Y} p_{Y|X=x}(y) L(y, f(x, z))
%\end{align}\label{f-g}
%Let $f^*(x, z) \in \mathcal A$ minimizes $\alpha(x, z)$, then we get
%\begin{align}
%f^*(x, z)=& \argmin_{f(x, z) \in \mathcal A} \sum_{y \in \mathcal Y} p_{Y|X=x}(y) L(y, f(x, z)) \nonumber\\
%=& \argmin_{a \in \mathcal A} \sum_{y \in \mathcal Y} p_{Y|X=x}(y) L(y, a) \nonumber\\
%=& \argmin_{g(x) \in \mathcal A} \sum_{y \in \mathcal Y} p_{Y|X=x}(y) L(y, g(x)),
%\end{align}
%where the last term is only a function of $x \in \mathcal X$. Hence, for all $x \in \mathcal X, z \in \mathcal Z$, there exists a function $f^* \in \Phi$ and a function $g^* \in \Psi$ such that $f^*(x, z)=g^*(x)$. 
%
%Because $Y \leftrightarrow X \leftrightarrow Z$ is a Markov chain, by using the definition of $L$-conditional entropy, we obtain
%\begin{align}\label{equality}
%H_L(Y | X, Z)=&\min_{f \in \Phi} \mathbb E_{Y, X, Z \sim P_{Y, X, Z}} [L(Y, f(X, Z))] \nonumber\\
%=&\min_{f \in \Phi} \sum_{y \in \mathcal Y, x \in \mathcal X, z \in \mathcal Z} P_{Y, X, Z}(y, x, z) L(y, f(x, z)) \nonumber\\
%=&\sum_{x \in \mathcal X, z \in \mathcal Z} P_{X, Z}(x, z) \min_{f(x, z) \in \mathcal A}\sum_{y \in \mathcal Y} P_{Y|X, Z}(y|x, z) L(y, f(x, z)) \nonumber\\
%\overset{(a)}{=}&\sum_{x \in \mathcal X, z \in \mathcal Z} P_{X, Z}(x, z) \min_{f(x, z) \in \mathcal A} \sum_{y \in \mathcal Y} P_{Y|X}(y|x) L(y, f(x, z)) \nonumber\\
%=&\sum_{x \in \mathcal X, z \in \mathcal Z}  P_{X, Z}(x, z) \sum_{y \in \mathcal Y} P_{Y|X}(y|x) L(y, f^*(x, z)) \nonumber\\
%\overset{(b)}{=}&\sum_{x \in \mathcal X, z \in \mathcal Z}  P_{X, Z}(x, z) \sum_{y \in \mathcal Y} P_{Y|X}(y|x) L(y, g^*(x)) \nonumber\\
%=&\sum_{x \in \mathcal X} P_X(x) \sum_{z \in \mathcal Z} P_{Z|X}(z|x) \sum_{y \in \mathcal Y} P_{Y|X}(y|x)  L(y, g^*(x)) \nonumber\\
%\overset{(c)}{=}&\sum_{x \in \mathcal X} P_X(x) \sum_{y \in \mathcal Y} P_{Y|X}(y|x) L(y, g^*(x)) \sum_{z \in \mathcal Z} P_{Z|X}(z|x) \nonumber\\
%\overset{(d)}{=}&\sum_{x \in \mathcal X} P_X(x) \sum_{y \in \mathcal Y} P_{Y|X}(y|x) L(y, g^*(x)) \nonumber\\
%=& \min_{g \in \Psi}  \mathbb E_{Y, X \sim P_{Y, X}} [L(Y, g(X))] \nonumber\\
%=&H_L(Y|X),
%\end{align}
%where the equality (a) is due to the Markov chain property, \eqref{f-g} yields (b), (c) holds because $L(y, g^*(x))$ does not depend on $Z$, and (d) is due to 
%\begin{align}
%\sum_{z \in \mathcal Z} P_{Z|X}(z|x) =1.
%\end{align}
%
%Equations \eqref{inequality} and \eqref{equality} yield \eqref{datainequality}. This concludes the proof of Lemma \ref{DataprocessingEn}.
%\end{proof}
%Because $\tilde Y_0 \leftrightarrow \tilde X_{-\theta, d_2} \leftrightarrow \tilde X_{-\theta, d_1}$ is a Markov chain, by using Lemma \ref{DataprocessingEn}, we obtain for all $\theta \in \mathcal D$, 
%\begin{align}\label{eqDataprocessing}
%H_L(\tilde Y_0| \tilde X_{-\theta, d_2}) \leq  H_L(\tilde Y_0| \tilde X_{-\theta, d_1}).
%\end{align}
%By using \eqref{eqDataprocessing} and \eqref{freshness_aware_cond}, we get
%\begin{align}
%H_L(\tilde Y_0| \tilde X_{-\Theta, d_2},\Theta) \leq H_L(\tilde Y_0| \tilde X_{-\Theta, d_1},\Theta).
%\end{align}
%This concludes the proof. 
%\end{proof}
%\subsubsection{Inference Error vs. Length of the Feature}
%\begin{lemma}\label{lemma_inference}
%If for all $x_d \in \mathcal X_d$,
%    \begin{align}\label{condition}
%    D_{\chi^2}\left(P_{Y_{t}|X_{t-\delta, d}=x_d} || P_{\tilde Y_0| \tilde X_{-\delta, d}=x_d}\right) \!\! \leq \beta^2,
%    \end{align}
%    then for all $1 \leq d_1 \leq d_2$
%    \begin{align}\label{Eq_lemma}
%       H_L(P_{Y_t|X_{t-\delta, d_2}}; P_{\tilde Y_0|\tilde X_{-\delta, d_2}}) \leq H_L(P_{Y_t|X_{t-\delta, d_1}}; P_{\tilde Y_0|\tilde X_{-\delta, d_1}})+O(\beta).
%    \end{align}
%\end{lemma}
%

